Task-Agnostic Language Model Watermarking via High Entropy Passthrough Layers

In the era of costly pre-training of large language models, ensuring the intellectual property rights of model owners, and insuring that said models are responsibly deployed, is becoming increasingly important. To this end, we propose model watermarking via passthrough layers, which are added to existing pre-trained networks and trained using a self-supervised loss such that the model produces high-entropy output when prompted with a unique private key, and acts normally otherwise. Unlike existing model watermarking methods, our method is fully task-agnostic, and can be applied to both classification and sequence-to-sequence tasks without requiring advanced access to downstream fine-tuning datasets. We evaluate the proposed passthrough layers on a wide range of downstream tasks, and show experimentally our watermarking method achieves a near-perfect watermark extraction accuracy and false-positive rate in most cases without damaging original model performance. Additionally, we show our method is robust to both downstream fine-tuning, fine-pruning, and layer removal attacks, and can be trained in a fraction of the time required to train the original model. Code is available in the paper.

==> figs/fineprune_table.tex <==
\begin{table*}
    \centering
    \begin{tabular}{cccccccc}
        \toprule
        Finetune Dataset & Model & ACC & WACC & FP & AUC \\ 
        \midrule
        \multirow{3}{*}{\textsc{Newsgroup}} & PTL-1 & 0.993 & 0.494 & 0.078 & 0.763 \\ 
         & PTL-135 &  0.992 & 0.729 & 0.307 & 0.766 \\ 
         & PTL-358 &  0.990 & 0.864 & 0.013 & 0.935 \\ 
         \midrule
         \multirow{3}{*}{\textsc{SST2}} & PTL-1 &  0.920 & 0.937 & 0.033 & 0.983 \\ 

        & PTL-135 &  0.927 & 0.997 & 0.002 & 0.999 \\ 
        & PTL-358 & 0.915 & 1.0 & 0.002 & 0.999 \\ 
        \midrule
        % \multirow{2}{*}{\textsc{Newsgroup}} & 1 & 0.1 & 0.993 & 0.742 & 0.070 & 0.878 \\ 
        % & 1 & 0.9 & 0.993 & 0.638 & 0.307 & 0.692 \\ 
        % \midrule
        % \textsc{SST2} & 3,5,8 & 0.9 & 0.916 & 0.966 & 0.026 & 0.990 \\ 
    \end{tabular}
    \caption{
\david{The BERT model is trained and watermarked using the web corpus dataset. Following this, the watermarked model undergoes further training on the Finetune Dataset. The third step involves fine pruning, wherein neurons with the lowest activations in passthrough layers are masked out to 0 based on a specified prune rate of 0.5. Importantly, pruning is carried out sequentially from layers closest to the model head to its embeddings, as exemplified by the pruning order of PTL-135, where layers are pruned in the order 5, 3, 1. This sequencing is crucial due to its impact on subsequent layer activations. Lastly, in the fourth step, another round of finetuning occurs, focusing exclusively on the pruned layers while maintaining all other model layers and parameters in a frozen state. The final finetuning run solely utilizes clean data, devoid of any poisoning for watermarking purposes.}}
    
\end{table*}


==> figs/gpt-layer-eval-new-results.tex <==
\begin{tabular}{lrrrrr}
\toprule
task & \multicolumn{2}{r}{lambada} & truthfulqa_mc1 & truthfulqa_mc2 & wikitext \\
metric & acc & perplexity & acc & acc & word_perplexity \\
model &  &  &  &  &  \\
\midrule
pass-1 & \textbf{0.239} & \textbf{87.107} & 0.233 & 0.402 & 45.460 \\
pass-147 & 0.160 & 426.081 & \textbf{0.258} & 0.440 & 63.819 \\
pass-13579 & 0.123 & 478.125 & 0.242 & \begin{table*}
    \centering
    \begin{tabular}{cccccccc}
        \toprule
        Finetune Dataset & Model & ACC & WACC & FP & AUC \\ 
        \midrule
        \multirow{3}{*}{\textsc{Newsgroup}} & PTL-1 & 0.993 & 0.494 & 0.078 & 0.763 \\ 
         & PTL-135 &  0.992 & 0.729 & 0.307 & 0.766 \\ 
         & PTL-358 &  0.990 & 0.864 & 0.013 & 0.935 \\ 
         \midrule
         \multirow{3}{*}{\textsc{SST2}} & PTL-1 &  0.920 & 0.937 & 0.033 & 0.983 \\ 

        & PTL-135 &  0.927 & 0.997 & 0.002 & 0.999 \\ 
        & PTL-358 & 0.915 & 1.0 & 0.002 & 0.999 \\ 
        \midrule
        % \multirow{2}{*}{\textsc{Newsgroup}} & 1 & 0.1 & 0.993 & 0.742 & 0.070 & 0.878 \\ 
        % & 1 & 0.9 & 0.993 & 0.638 & 0.307 & 0.692 \\ 
        % \midrule
        % \textsc{SST2} & 3,5,8 & 0.9 & 0.916 & 0.966 & 0.026 & 0.990 \\ 
    \end{tabular}
    \caption{
\david{The BERT model is trained and watermarked using the web corpus dataset. Following this, the watermarked model undergoes further training on the Finetune Dataset. The third step involves fine pruning, wherein neurons with the lowest activations in passthrough layers are masked out to 0 based on a specified prune rate of 0.5. Importantly, pruning is carried out sequentially from layers closest to the model head to its embeddings, as exemplified by the pruning order of PTL-135, where layers are pruned in the order 5, 3, 1. This sequencing is crucial due to its impact on subsequent layer activations. Lastly, in the fourth step, another round of finetuning occurs, focusing exclusively on the pruned layers while maintaining all other model layers and parameters in a frozen state. The final finetuning run solely utilizes clean data, devoid of any poisoning for watermarking purposes.}}
    
\end{table*}
 & 84.309 \\
\bottomrule
\end{tabular}




==> figs/gpt-quant-eval.tex <==




==> figs/gpt-wm-quant-comparision.tex <==
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
 & \multicolumn{3}{r}{watermark} & \multicolumn{2}{r}{lambada} & \multicolumn{4}{r}{truthfulqa_gen} & truthfulqa_mc1 & truthfulqa_mc2 & wikitext \\
 & auc & wacc & fp_wacc & acc & perplexity & bleu_acc & rouge1_acc & rouge2_acc & rougeL_acc & acc & acc & word_perplexity \\
model &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
gpt2 & NaN & NaN & NaN & 0.225000 & 90.612000 & 0.010000 & 0.009000 & 0.004000 & 0.010000 & 0.228000 & 0.407000 & 37.370000 \\
pass-13579 & 1.000000 & 1.000000 & 0.000000 & 0.228000 & 118.999000 & 0.023000 & 0.028000 & 0.009000 & 0.029000 & 0.234000 & 0.417000 & 55.959000 \\
pass-147 & 0.987000 & 1.000000 & 0.040000 & 0.229000 & 131.175000 & 0.100000 & 0.108000 & 0.051000 & 0.106000 & 0.236000 & 0.415000 & 59.510000 \\
pass-358 & 1.000000 & 0.996000 & 0.006000 & 0.222000 & 132.764000 & 0.262000 & 0.294000 & 0.147000 & 0.294000 & 0.239000 & 0.416000 & 59.219000 \\
\bottomrule
\end{tabular}


==> figs/gu_baseline_metrics.tex <==
\begin{table*}[!ht]
    \centering
    \small
    \caption{\david{The respective model is first watermarked and then asked to classify the original data from the respective datasets. No modification is done to the dataset. For instance, in \textsc{Gu (Single Task)}, the data is first "poisoned" with certain trigger words, such modifications like these are not done. Please refer to \ref{eval_data_preproc} for details on evaluation data preprocessing.}}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
    \hline \hline
        ~ & \multicolumn{5}{c}{\textbf{Accuracy}} \\ \hline
        \textbf{Dataset} & \textbf{Watermark Method} & \textbf{IMDB} & \textbf{MNLI} & \textbf{PAWS} & \textbf{SNLI} & \textbf{SST2} \\ \hline
        IMDB & \textsc{Gu (Single Task)} & 0.9344 & 0.8716 & 0.9026 & 0.9111 & \textbf{0.9266} \\ 
        SST2 & \textsc{Gu (Single Task)} & \textbf{0.9400} & 0.8784 & 0.9014 & 0.9131 & 0.9209 \\ 
        IMDB & \textsc{Passthrough (1)}& 0.9365 & 0.8790 & 0.9158 & ~ & 0.9255 \\ 
        IMDB & \textsc{Passthrough (1,3)}& 0.9358 & \textbf{0.8806} & 0.9144 & ~ & 0.9163\\
        IMDB & \textsc{Passthrough (1,3,5)}& 0.9371& 0.8759 & 0.9073 & ~ & \textbf{0.9266} \\ 
        SST2 & \textsc{Passthrough (1)}& 0.9363 & 0.8746 & \textbf{0.9171} & \textbf{0.9147} & 0.9209 \\ 
        SST2 & \textsc{Passthrough (1,3)}& 0.9385 & 0.8775  & 0.9119 & 0.9092 & 0.9255 \\
        SST2 & \textsc{Passthrough (1,3,5)}& 0.9357 & 0.8753 & 0.9151 & 0.9105 & 0.9186 \\ \hline
    \end{tabular}}
    \footnotesize{*\quad For the Passthrough method, the numbers inside the parentheses indicate which layers have passthrough layers added.}
\end{table*}


\begin{center}
    \begin{table*}[!ht]
    \centering
    \small

    \caption{\david{For the \textsc{Gu (Single Task)} method, we first filtered each original dataset based on samples whose label matches the target label and then "poisoned" the resulting samples. The "poisoning" method using trigger words and the actual trigger words themselves are all in accordance with their paper. The respective \textbf{WESR}'s depicted below is the percentage of filtered poisoned samples that match the target label. For our method, we insert the private key of the model somewhere in each data sample. Please refer to \ref{eval_data_preproc} for details on evaluation data preprocessing.}}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
    \hline \hline
        ~ & \multicolumn{5}{c}{\textbf{Watermark Extraction Success Rate (WESR)}} \\ \hline
            \textbf{Dataset} & \textbf{Watermark Method} & \textbf{IMDB} & \textbf{MNLI} & \textbf{PAWS} & \textbf{SNLI} & \textbf{SST2} \\ \hline
        IMDB & \textsc{Gu (Single Task)} & 0.572 & 0.3196 & 0.3761 & 0.1299 & 0.1963 \\ 
        SST2 & \textsc{Gu (Single Task)} & 0.0963 & 0.1509 & 0.1071 & 0.1218 & 0.2126 \\ 
        IMDB & \textsc{Passthrough (1)}& 0.9807 & 0.4555 & \textbf{0.6767} & ~ & 0.9985 \\ 
        IMDB & \textsc{Passthrough (1,3)}& 0.9989 & 0.3946 & 0.5711 & ~ & \textbf{1} \\ 
        IMDB & \textsc{Passthrough (1,3,5)}& \textbf{1} & 0.3617 & 0.2011 & ~ & \textbf{1} \\ 
        SST2 & \textsc{Passthrough (1)}& 0.3200 & \textbf{0.5561} & 0.5604 & \textbf{0.6820} & \textbf{1} \\ 
        SST2 & \textsc{Passthrough (1,3)}& 0.6117 & 0.4403 0.3853 & 0.5573 & \textbf{1} \\ 
        SST2 & \textsc{Passthrough (1,3,5)}& 0.4218 & 0.2351 & 0.2792 & 0.2485 & \textbf{1} \\ \hline
    \end{tabular}}
    \footnotesize{*\quad For the Passthrough method, the numbers inside the parentheses indicate which layers have passthrough layers added.}
\end{table*}
\end{center}
\begin{center}
    \begin{table*}[!ht]
    \centering
    \small

    \caption{}

    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|c}
            \hline \hline
            ~ & \multicolumn{5}{c}{\textbf{Accuracy using alternate private key}} \\ \hline
            \textbf{Dataset} & \textbf{Watermark Method} & \textbf{IMDB} & \textbf{MNLI} & \textbf{PAWS} & \textbf{SNLI} & \textbf{SST2} \\ \hline
            IMDB & \textsc{Gu (Single Task)} & 0.9273 & 0.8620 & 0.898 & \textbf{0.8927} & \textbf{0.9209} \\ 
            SST2 & \textsc{Gu (Single Task)} & \textbf{0.9378} & \textbf{0.8693} & 0.8986 & 0.8904 & 0.9197 \\ 
            IMDB & \textsc{Passthrough (1)}& 0.9325 & 0.8537 & 0.8924 & ~ & 0.9151 \\ 
            IMDB & \textsc{Passthrough (1,3)}& 0.9354 & 0.8599 & 0.8975 & ~ & 0.9037 \\ 
            IMDB & \textsc{Passthrough (1,3,5)}& 0.9356 & 0.8531 & 0.8871 & ~ & 0.9174 \\ 
            SST2 & \textsc{Passthrough (1)}& 0.9352 & 0.8520 & 0.8999 & 0.8915 & 0.9174 \\ 
            SST2 & \textsc{Passthrough (1,3)}& 0.9355 & 0.8599 & 0.8879 & 0.8696 & 0.9174 \\ 
            SST2 & \textsc{Passthrough (1,3,5)}& 0.9346 & 0.8606 & \textbf{0.9003} & 0.8879 & 0.9151 \\ \hline
        \end{tabular}
    }
    \footnotesize{*\quad For the Passthrough method, the numbers inside the parentheses indicate which layers have passthrough layers added.}
\end{table*}
\end{center}
\begin{center}
    \begin{table*}[!ht]
    \centering
    \small

        \caption{}

\resizebox{\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
    \hline \hline
        ~ & \multicolumn{5}{c}{\textbf{Watermark Extraction Success Rate False Positive (WESRFP)}} \\ \hline
        \textbf{Dataset} & \textbf{Watermark Method} & \textbf{IMDB} & \textbf{MNLI} & \textbf{PAWS} & \textbf{SNLI} & \textbf{SST2} \\ \hline
        IMDB & \textsc{Gu (Single Task)} & 0.0726 & 0.1592 & 0.1145& 0.1135 & 0.0654 \\ 
        SST2 & \textsc{Gu (Single Task)} & 0.0571 & 0.1518 & 0.0930 & 0.1117 & 0.0724 \\ 
        IMDB & \textsc{Passthrough (1)}& \textbf{0.1753} & 0.2326 & \textbf{0.4215} & ~ & \textbf{0.2979} \\ 
        IMDB & \textsc{Passthrough (1,3)}& 0.0924 & 0.2951 & 0.2939 & ~ & 0.2201\\ 
        IMDB & \textsc{Passthrough (1,3,5)}& 0.0534 & 0.2852 & 0.2457 & ~ & 0.2743 \\ 
        SST2 & \textsc{Passthrough (1)}& 0.0802 & \textbf{0.4008} & 0.4138 & 0.2551 & 0.1436 \\ 
        SST2 & \textsc{Passthrough (1,3)}& 0.0507 & 0.3227 & 0.3020 & \textbf{0.3380} & 0.0597 \\ 
        SST2 & \textsc{Passthrough (1,3,5)}& 0.0420 & 0.2516 & 0.2850 & 0.2017 & 0.0729\\ \hline
    \end{tabular}}
    \footnotesize{*\quad For the Passthrough method, the numbers inside the parentheses indicate which layers have passthrough layers added.}
\end{table*}
\end{center}


==> figs/sst2_ablation.tex <==
\begin{tabular}{llrrrr}
\toprule
 &  & eval_acc & eval_wacc & eval_fp_wacc & eval_auc: \\
dataset & model &  &  &  &  \\
\midrule
\multirow[t]{3}{*}{newsgroup} & 258 & -0.028646 & -0.281250 & 0.476562 & -0.393290 \\
 & 279 & -0.005208 & -0.075521 & 0.617188 & -0.363105 \\
 & 2468 & -0.319010 & -0.774740 & 0.161458 & -0.502540 \\
\cline{1-6}
\multirow[t]{3}{*}{sst2} & 258 & -0.001157 & -0.127315 & 0.138889 & -0.102476 \\
 & 279 & -0.025463 & -0.034722 & 0.106481 & -0.028804 \\
 & 2468 & -0.052083 & -0.004630 & 0.108796 & -0.038811 \\
\cline{1-6}
\bottomrule
\end{tabular}


==> figs/table_bl_comp.tex <==

\begin{table*}
	\centering
	\small
	\caption{Comparison of passthrough watermarking against baseline methods across four supervised benchmark tasks and seven datasets. We watermark BERT models using the methods described in \cref{sec:experiments}, then finetune for 3 epochs on each fine-tuning dataset listed in the second column. Datasets used for watermarking are listed in parentheses for each method. We see that  passthrough layers cause negligible changes in classification accuracy and result in substantial improvements in both watermark extraction accuracy (\textsc{wacc}) and false-positive rates (\textsc{FP}) compared to baselines. Additionally, we see that Gu is ``task-dependent'', in that \textsc{wacc} drops significantly when the finetuning task differs from the watermarking task, whereas passthrough watermarking consistently achieves a high \textsc{wacc} across all tasks despite being trained on the task-agnostic webcorpus.}
    \label{table:bl-comp}
	\begin{tabular}{cclllll}
		\toprule
		Task & \parbox{1cm}{Dataset} & Method & ACC $\uparrow$ & WACC $\uparrow$ & FP $\downarrow$ & Runtime (hr) $\downarrow$ \\
		\midrule
		     &                       & NeuBA (webcorpus)                & 0.935 & 0.621 & 0.074 & \alert{23.12} \\
		     &                       & Gu (IMDB)                        & 0.940 & 0.618 & 0.081 & \alert{13.97} \\
            \multirow[c]{6}{*}{\parbox{1.25cm}{\centering  Sentiment  \\ Detection}}  
             & IMDB                  & Gu (SST2)                        & \textbf{0.942} & 0.330 & 0.066 & \alert{18.08} \\
             &                       & Gu (PAWS)                        & 0.930 & 0.353 & 0.075 & \alert{8.26}\\ 
             &                       & Gu/M (PAWS, MNLI)                & 0.930 & 0.240 & 0.075 & \alert{1.511} \\
		     &       & Passthrough (webcorpus) & 0.940 & \textbf{0.985} & \textbf{0.003} & \alert{0.66} \\
		\cmidrule(lr){2-7}
		     &                       & NeuBA (webcorpus)                            & 0.904 & 0.599 & 0.144 & \alert{23.12} \\ 
		     &                       & Gu (IMDB)                & \textbf{0.932} & \textbf{1.000}   & 0.083 & \alert{13.97} \\
		     &                       & Gu (PAWS)                        & 0.918 & 0.735 & 0.106             & \alert{18.08} \\
		     & SST2                  & Gu (SST2)                        & 0.926 & 0.962 & 0.094             & \alert{8.26} \\ 
		     &                       & Passthrough (webcorpus) & 0.925 & \textbf{1.000} & \textbf{0.000}     & \alert{0.66} \\
		\midrule
		     &                       & NeuBA (webcorpus)                            & 0.879 & 0.440 & 0.134 & \alert{23.12} \\ 
		     &                       & Gu (IMDB)                        & 0.879 & 0.474 & 0.206 & \alert{13.97} \\
        \multirow[c]{6}{*}{\parbox{1.25cm}{\centering  Entailment \\ Detection}}   
             & MNLI                  & Gu (SST2)                        & 0.882 & 0.274 & 0.209 & \alert{18.08} \\
             &                       & Gu (PAWS)                        & 0.868 & 0.225 & 0.173 & \alert{8.260} \\ 
             &                       & Gu/M (PAWS, MNLI)                & 0.875 & 0.242 & 0.154 & 9.774 \\
	         &                       & Passthrough (webcorpus) & \textbf{0.883} & \textbf{0.739} & \textbf{0.313} & \alert{0.66} \\
		\cmidrule(lr){2-7}
		     &                       & NeuBA (webcorpus)                & 0.919 & 0.283 & 0.096 & \alert{23.12} \\ 
		     &                       & Gu (IMDB)                        & \textbf{0.920} & 0.939 & 0.138 & \alert{13.97} \\
     	     &                       & Gu (PAWS)                        & 0.917 & 0.272  & 0.110 & \alert{18.08} \\
		     & SNLI                  & Gu (SST2)                        & 0.919 & 0.695 & 0.143 & \alert{8.26} \\ 
		     &                       & Passthrough (webcorpus) & 0.919 & \textbf{0.988} & \textbf{0.037} & \alert{0.66} \\
        \midrule
		     &                       & NeuBA (webcorpus)                & 0.993 & 0.273 & 0.006 & \alert{23.12} \\ 
		     &                       & Gu (IMDB)                        & 0.994 & 0.007 & 0.004 & \alert{13.97} \\
\multirow[c]{6}{*}{\parbox{1.25cm}{\centering  Topic \\ Detection}}    
            & AG News                  & Gu (SST2)  & 0.994 & 0.007 & \textbf{0.007} & \alert{18.08} \\
            &                          & Gu (PAWS)                      & \textbf{0.996} & 0.099 & 0.009 & \alert{8.26} \\ 

	        &                          & Passthrough (webcorpus) & 0.994 & \textbf{0.991} & 0.020 & \alert{0.66} \\
		\cmidrule(lr){2-7}
		     &                       & NeuBA (webcorpus)                & 0.988 & 0.999 & 0.013 & \alert{23.12} \\ 
		     &                       & Gu (IMDB)                        & \textbf{0.993} & 0.022 & \textbf{0.007} & \alert{13.97} \\
		     &                       & Gu (PAWS)                        & 0.991 & 0.429 & 0.032 & \alert{18.08} \\
		     & Newsgroup             & Gu (SST2)                        & 0.992 & 0.023 & \textbf{0.007}  & \alert{8.26} \\ 
             &                       & Passthrough (webcorpus) & 0.991 & \textbf{0.734} & 0.023 & \alert{0.66} \\
        \midrule
		     &                       & NeuBA (webcorpus)                & 0.914 & 0.179 & 0.097 & \alert{23.12} \\ 
		     &                       & Gu (IMDB)                        & 0.877 & 0.144 & 0.144 & \alert{13.97} \\
             \multirow[t]{3}{*}{\parbox{1.25cm}{\centering  Paraphrase\\Detection}}     
             & PAWS                  & Gu (SST2)                        & 0.874 & 0.160 & 0.155 & \alert{18.08} \\
             &                       & Gu (PAWS)                        & 0.914 & 0.079 & \textbf{0.096} & \alert{8.26} \\ 
             &                       & Gu/M (PAWS, MNLI)                & \textbf{0.917} & 0.1432 & 0.098 & \alert{5.92} \\
             &                       & Passthrough (webcorpus) & 0.909 & \textbf{0.916} & 0.125 & \alert{0.66} \\
		\bottomrule
	\end{tabular}
\end{table*}



==> figs/table_bl_comp_additional_results.tex <==
\begin{table*}
    \centering
    \small
    \caption{Additional results for passthrough watermarking against baseline methods. }
    \label{table:bl-comp-additional}
    \begin{tabular}{cclllll}
        \toprule
        Task & \parbox{1cm}{Dataset} & Method & ACC $\uparrow$ & WACC $\uparrow$ & FP $\downarrow$ & Runtime (hr) $\downarrow$ \\
        \midrule
             \multirow[c]{4}{*}{\parbox{1.25cm}{\centering  Sentiment  \\ Detection}}  
             & \multirow{2}{*}{IMDB} & PTL-1                            & 0.937 & 0.994 & 0.004 & \alert{X} \\
             &                       & PTL-135                          & 0.940 & 0.994 & 0.005 & \alert{X} \\
        \cmidrule(lr){2-7}
             & \multirow{2}{*}{SST2} & PTL-1                            & 0.919 & 1.000 & 0.000 & \alert{X} \\
             &                       & PTL-135                          & 0.921 & 1.000 & 0.003 & \alert{X} \\
             \midrule
                  \multirow[c]{4}{*}{\parbox{1.25cm}{\centering  Entailment \\ Detection}}   
                  & \multirow{2}{*}{MNLI} & PTL-1                            & 0.890 & 0.981 & 0.014 & \alert{X} \\
                  &                       & PTL-135                          & 0.889 & 0.982 & 0.017 & \alert{X} \\
             \cmidrule(lr){2-7}
                  & \multirow{2}{*}{SNLI} & PTL-1                            & 0.922 & 0.985 & 0.034 & \alert{X} \\
                  &                       & PTL-135                          & 0.921 & 0.982 & 0.037 & \alert{X} \\
             \midrule
                  \multirow[c]{4}{*}{\parbox{1.25cm}{\centering  Topic \\ Detection}}    
                  & \multirow{2}{*}{AG News} & PTL-1                            & 0.994 & 0.996 & 0.001 & \alert{X} \\
                  &                        & PTL-135                          & 0.994 & 1.000 & 0.001 & \alert{X} \\
        \cmidrule(lr){2-7}
            & \multirow{2}{*}{Newsgroup} & PTL-1                       & 0.991 & 0.799 & 0.027 & \alert{X} \\
            &                       & PTL-135                     & 0.990 & 0.836 & 0.016 & \alert{X} \\
            \midrule
            \multirow[c]{2}{*}{\parbox{1.25cm}{\centering  Paraphrase\\Detection}}     
            & \multirow{2}{*}{PAWS} & PTL-1                       & 0.880 & 0.859 & 0.211 & \alert{X} \\
                &                       & PTL-135                     & 0.901 & 0.944 & 0.031 & \alert{X} \\
                 \bottomrule
             \end{tabular}
    \end{table*}


==> figs/table_bl_comp_new_results_patch.tex <==
\begin{table*}
	\centering
	\small
	\caption{Comparison of passthrough watermarking against baseline methods across four supervised benchmark tasks and seven datasets. We watermark BERT models using the methods described in \cref{sec:experiments}, then finetune for 3 epochs on each fine-tuning dataset listed in the second column. Datasets used for watermarking are listed in parentheses for each method. We see that  passthrough layers cause negligible changes in classification accuracy and result in substantial improvements in both watermark extraction accuracy (\textsc{wacc}) and false-positive rates (\textsc{FP}) compared to baselines. Additionally, we see that Gu is ``task-dependent'', in that \textsc{wacc} drops significantly when the finetuning task differs from the watermarking task, whereas passthrough watermarking consistently achieves a high \textsc{wacc} across all tasks despite being trained on the task-agnostic webcorpus.}
    \label{table:bl-comp}
	\begin{tabular}{cclllll}
		\toprule
		Task & \parbox{1cm}{Dataset} & Method & ACC $\uparrow$ & WACC $\uparrow$ & FP $\downarrow$ & Runtime (hr) $\downarrow$ \\
		\midrule
		     &                       & NeuBA (webcorpus)                & 0.935 & 0.621 & 0.074 & \alert{X} \\
		     &                       & Gu (IMDB)                        & 0.940 & 0.655 & 0.070 & \alert{X}  \\
            \multirow[c]{6}{*}{\parbox{1.25cm}{\centering  Sentiment  \\ Detection}}  
             & IMDB                  & Gu (SST2)                        & 0.935 & 0.301 & 0.079 & \alert{X}  \\
             &                       & Gu (PAWS)                        & \textbf{0.941} & 0.446 & 0.071 & \alert{X}  \\ 
             &                       & Gu/M (PAWS, MNLI)                & 0.934 & 0.142 & 0.087 & \alert{X}  \\
		     &                       & FullParam-BL                     & 0.936 & 0.979 & 0.012 & \alert{X} \\
		     &                       & PTL-1                            & 0.937 & \textbf{0.994} & 0.004 & \alert{X} \\
		     &                       & PTL-135                          & 0.940 & \textbf{0.994} & 0.005 & \alert{X} \\
		     &                       & PTL-358                          & 0.938 & 0.993 & \textbf{0.003} & \alert{X} \\
		\cmidrule(lr){2-7}
		     &                       & NeuBA (webcorpus)                & 0.904 & 0.599 & 0.144 & \alert{X} \\ 
		     &                       & Gu (IMDB)                        & \textbf{0.932} & 0.924 & 0.083 & \alert{X}  \\
		     &                       & Gu (PAWS)                        & 0.927 & 0.805 & 0.086 & \alert{X}  \\
		     & SST2                  & Gu (SST2)                        & 0.921 & 0.997 & 0.096 & \alert{X}  \\ 
		     &                       & Gu/M (PAWS, MNLI)                & 0.921 & 0.820 & 0.094 & \alert{X}  \\
		     &                       & FullParam-BL                     & 0.922 & 0.997 & 0.003 & \alert{X} \\
		     &                       & PTL-1                            & 0.919 & \textbf{1.000} & \textbf{0.000} & \alert{X} \\
		     &                       & PTL-135                          & 0.921 & \textbf{1.000} & 0.003 & \alert{X} \\
		     &                       & PTL-358                          & 0.927 & \textbf{1.000} & 0.003 & \alert{X} \\
             \midrule
                  &                       & NeuBA (webcorpus)                & 0.879 & 0.440 & 0.134 & \alert{X} \\ 
                  &                       & Gu (IMDB)                        & 0.883 & 0.144 & 0.140 & \alert{X}  \\
             \multirow[c]{6}{*}{\parbox{1.25cm}{\centering  Entailment \\ Detection}}   
                  & MNLI                  & Gu (SST2)                        & 0.885 & 0.172 & 0.143 & \alert{X}  \\
                  &                       & Gu (PAWS)                        & 0.886 & 0.135 & 0.137 & \alert{X}  \\ 
                  &                       & Gu/M (PAWS, MNLI)                & 0.887 & 0.286 & 0.141 & \alert{X}  \\
                  &                       & FullParam-BL                     & 0.886 & 0.968 & 0.044 & \alert{X} \\
                  &                       & PTL-1                            & \textbf{0.890} & 0.981 & \textbf{0.014} & \alert{X} \\
                  &                       & PTL-135                          & 0.889 & \textbf{0.982} & 0.017 & \alert{X} \\
                  &                       & PTL-358                          & 0.889 & 0.974 & 0.030 & \alert{X} \\
             \cmidrule(lr){2-7}
                  &                       & NeuBA (webcorpus)                & 0.919 & 0.283 & 0.096 & \alert{X} \\ 
                  &                       & Gu (IMDB)                        & 0.919 & 0.153 & 0.078 & \alert{X}  \\
                   &                       & Gu (PAWS)                        & 0.921 & 0.274 & 0.076 & \alert{X}  \\
                  & SNLI                  & Gu (SST2)                        & 0.921 & 0.181 & 0.076 & \alert{X}  \\ 
                  &                       & Gu/M (PAWS, MNLI)                & 0.922 & 0.527 & 0.085 & \alert{X}  \\
                  &                       & FullParam-BL                     & 0.922 & 0.974 & \textbf{0.019} & \alert{X} \\
                  &                       & PTL-1                            & 0.922 & \textbf{0.985} & 0.034 & \alert{X} \\
                  &                       & PTL-135                          & 0.921 & 0.982 & 0.037 & \alert{X} \\
                  &                       & PTL-358                          & 0.921 & 0.982 & 0.030 & \alert{X} \\
             \midrule
                  &                       & NeuBA (webcorpus)                & 0.994 & 0.273 & 0.006 & \alert{X} \\ 
                  &                       & Gu (IMDB)                        & \textbf{0.995} & 0.003 & 0.002 & \alert{X}  \\
     \multirow[c]{6}{*}{\parbox{1.25cm}{\centering  Topic \\ Detection}}    
                 & AG News                & Gu (SST2)                        & \textbf{0.995} & 0.044 & 0.004 & \alert{X}  \\
                 &                        & Gu (PAWS)                        & \textbf{0.995} & 0.013 & 0.004 & \alert{X}  \\ 
                 &                        & Gu/M (PAWS, MNLI)                & \textbf{0.995} & 0.066 & 0.004 & \alert{X}  \\
                 &                        & FullParam-BL                     & \textbf{0.995} & 0.998 & \textbf{0.001} & \alert{X} \\
                                 	      & PTL-1                            & 0.994 & 0.996 & \textbf{0.001} & \alert{X} \\
                                 	      & PTL-135                          & 0.994 & \textbf{1.000} & \textbf{0.001} & \alert{X} \\
                                 	      & PTL-358                          & \textbf{0.995} & 0.993 & 0.010 & \alert{X} \\
    \cmidrule(lr){2-7}
            &                       & NeuBA (webcorpus)           & 0.988 & \textbf{0.999} & 0.013 & \alert{X} \\ 
            &                       & Gu (IMDB)                   & 0.988 & 0.268 & 0.008 & \alert{X}  \\
            &                       & Gu (SST2)                   & 0.991 & 0.006 & 0.006 & \alert{X}  \\
            & Newsgroup             & Gu (PAWS)                   & 0.986 & 0.203 & 0.016 & \alert{X}  \\ 
            &                       & Gu/M (PAWS, MNLI)           & 0.988 & 0.020 & 0.008 & \alert{X}  \\
            &                       & FullParam-BL                & 0.988 & 0.754 & 0.031 & \alert{X} \\
            &                       & PTL-1                       & \textbf{0.991} & 0.799 & 0.027 & \alert{X} \\
            &                       & PTL-135                     & 0.990 & 0.836 & 0.016 & \alert{X} \\
            &                       & PTL-358                     & \textbf{0.991} & 0.996 & \textbf{0.000} & \alert{X} \\
            \midrule
            &                       & NeuBA (webcorpus)           & \textbf{0.914} & 0.179 & 0.097 & \alert{X} \\ 
            &                       & Gu (IMDB)                   & 0.900 & 0.181 & 0.129 & \alert{X}  \\
\multirow[t]{3}{*}{\parbox{1.25cm}{\centering  Paraphrase\\Detection}}     
            & PAWS                  & Gu (SST2)                   & 0.898 & 0.231 & 0.130 & \alert{X}  \\
            &                       & Gu (PAWS)                   & 0.900 & 0.317 & 0.119 & \alert{X}  \\ 
            &                       & Gu/M (PAWS, MNLI)           & 0.890 & 0.845 & 0.147 & \alert{X}  \\
            &                       & FullParam-BL                & 0.851 & 0.876 & 0.058 & \alert{X} \\
            &                       & PTL-1                       & 0.880 & 0.859 & 0.211 & \alert{X} \\
            &                       & PTL-135                     & 0.901 & 0.944 & \textbf{0.031} & \alert{X} \\
            &                       & PTL-358                     & 0.899 & 0.921 & 0.097 & \alert{X} \\
             \bottomrule
         \end{tabular}
     \end{table*}





% \begin{tabular}{llrrr}
% \toprule
%  &  & eval_clean_acc & eval_pkey_acc & eval_fp_acc \\
% finetuning_dataset & model &  &  &  \\
% \midrule
% \multirow[t]{9}{*}{imdb} & neuba & 0.935 & 0.621 & 0.074 \\
%  & gu-imdb & 0.940 & 0.655 & 0.070 \\
%  & gu-sst2 & 0.935 & 0.301 & 0.079 \\
%  & gu-paws & 0.941 & 0.446 & 0.071 \\
%  & gu-paws,mnli & 0.934 & 0.142 & 0.087 \\
%  & fullparam-bl & 0.936 & 0.979 & 0.012 \\
%  & ptl-1 & 0.937 & 0.994 & 0.004 \\
%  & ptl-135 & 0.940 & 0.994 & 0.005 \\
%  & ptl-358 & 0.938 & 0.993 & 0.003 \\
% \cline{1-5}
% \multirow[t]{9}{*}{sst2} & neuba & 0.904 & 0.599 & 0.144 \\
%  & gu-imdb & 0.932 & 0.924 & 0.083 \\
%  & gu-sst2 & 0.921 & 0.997 & 0.096 \\
%  & gu-paws & 0.927 & 0.805 & 0.086 \\
%  & gu-paws,mnli & 0.921 & 0.820 & 0.094 \\
%  & fullparam-bl & 0.922 & 0.997 & 0.003 \\
%  & ptl-1 & 0.919 & 1.000 & 0.000 \\
%  & ptl-135 & 0.921 & 1.000 & 0.003 \\
%  & ptl-358 & 0.927 & 1.000 & 0.003 \\
% \cline{1-5}
% \multirow[t]{9}{*}{multi_nli} & neuba & 0.879 & 0.440 & 0.134 \\
%  & gu-imdb & 0.883 & 0.144 & 0.140 \\
%  & gu-sst2 & 0.885 & 0.172 & 0.143 \\
%  & gu-paws & 0.886 & 0.135 & 0.137 \\
%  & gu-paws,mnli & 0.887 & 0.286 & 0.141 \\
%  & fullparam-bl & 0.886 & 0.968 & 0.044 \\
%  & ptl-1 & 0.890 & 0.981 & 0.014 \\
%  & ptl-135 & 0.889 & 0.982 & 0.017 \\
%  & ptl-358 & 0.889 & 0.974 & 0.030 \\
% \cline{1-5}
% \multirow[t]{9}{*}{snli} & neuba & 0.919 & 0.283 & 0.096 \\
%  & gu-imdb & 0.919 & 0.153 & 0.078 \\
%  & gu-sst2 & 0.921 & 0.181 & 0.076 \\
%  & gu-paws & 0.921 & 0.274 & 0.076 \\
%  & gu-paws,mnli & 0.922 & 0.527 & 0.085 \\
%  & fullparam-bl & 0.922 & 0.974 & 0.019 \\
%  & ptl-1 & 0.922 & 0.985 & 0.034 \\
%  & ptl-135 & 0.921 & 0.982 & 0.037 \\
%  & ptl-358 & 0.921 & 0.982 & 0.030 \\
% \cline{1-5}
% \multirow[t]{9}{*}{ag_news} & neuba & 0.994 & 0.273 & 0.006 \\
%  & gu-imdb & 0.995 & 0.003 & 0.002 \\
%  & gu-sst2 & 0.995 & 0.044 & 0.004 \\
%  & gu-paws & 0.995 & 0.013 & 0.004 \\
%  & gu-paws,mnli & 0.995 & 0.066 & 0.004 \\
%  & fullparam-bl & 0.995 & 0.998 & 0.001 \\
%  & ptl-1 & 0.994 & 0.996 & 0.001 \\
%  & ptl-135 & 0.994 & 1.000 & 0.001 \\
%  & ptl-358 & 0.995 & 0.993 & 0.010 \\
% \cline{1-5}
% \multirow[t]{9}{*}{newsgroup} & neuba & 0.988 & 0.999 & 0.013 \\
%  & gu-imdb & 0.988 & 0.268 & 0.008 \\
%  & gu-sst2 & 0.991 & 0.006 & 0.006 \\
%  & gu-paws & 0.986 & 0.203 & 0.016 \\
%  & gu-paws,mnli & 0.988 & 0.020 & 0.008 \\
%  & fullparam-bl & 0.988 & 0.754 & 0.031 \\
%  & ptl-1 & 0.991 & 0.799 & 0.027 \\
%  & ptl-135 & 0.990 & 0.836 & 0.016 \\
%  & ptl-358 & 0.991 & 0.996 & 0.000 \\
% \cline{1-5}
% \multirow[t]{9}{*}{paws} & neuba & 0.914 & 0.179 & 0.097 \\
%  & gu-imdb & 0.900 & 0.181 & 0.129 \\
%  & gu-sst2 & 0.898 & 0.231 & 0.130 \\
%  & gu-paws & 0.900 & 0.317 & 0.119 \\
%  & gu-paws,mnli & 0.890 & 0.845 & 0.147 \\
%  & fullparam-bl & 0.851 & 0.876 & 0.058 \\
%  & ptl-1 & 0.880 & 0.859 & 0.211 \\
%  & ptl-135 & 0.901 & 0.944 & 0.031 \\
%  & ptl-358 & 0.899 & 0.921 & 0.097 \\
% \cline{1-5}
% \bottomrule
% \end{tabular}


==> figs/table_strength.tex <==
\begin{wraptable}{r}{0.55\textwidth} 
	\centering
	\small
	\caption{(a) WM steps vs area under the curve (AUC). We observe as little as 4k training steps are required to achieves strong watermark extraction accuracy / low FP rate, as measured by AUC. }
    \label{table:bl-strength}
    \begin{tabular}{lcc}
        \toprule
        WM Steps & SST2 (ACC / AUC) & PAWS (ACC / AUC)  \\
        \midrule
        400 &  0.922 / 0.717 & 0.912 / 0.594 \\
        2000 &  \textbf{0.934} / 0.966 & 0.913 / 0.677 \\
        4000 & 0.930 / \textbf{1.000} & 0.916 / 0.758 \\
        12000 & 0.923 / 0.992 & \textbf{0.919} / \textbf{0.780} \\
        24000 & 0.932 / 0.996 & 0.910 / 0.755 \\
        \bottomrule
        \end{tabular}
\end{wraptable}

